Supporting Sensemaking of Large Language Model Outputs at Scale

Large language models (LLMs) are capable of generating multiple responses to a single prompt, yet little effort has been expended to help end-users or system designers make use of this capability. In this paper, we explore how to present many LLM responses at once. We design five features, which include both pre-existing and novel methods for computing similarities and differences across textual documents, as well as how to render their outputs. We report on a controlled user study (n=24) and eight case studies evaluating these features and how they support users in different tasks. We find that the features support a wide variety of sensemaking tasks and even make tasks previously considered to be too difficult by our participants now tractable. Finally, we present design guidelines to inform future explorations of new LLM interfaces.

==> sections/codebook.tex <==

    
  \begin{tabular}{lp{12cm}}
    \toprule
    Code & Definition\\
    \midrule
    \multicolumn{2}{l}{\textbf{Kinds of Similarities and Differences Noticed}} \\

        style
        & Stylistic or tone similarities and differences.
        \\
        content
        & Content similarities and differences, including counting phrases and the length of responses.
        \\
        granularity
        & Level of abstraction of similarities and differences, e.g. high level v. low level or  “granularity”.
        \\
        structure
        & Structural similarities and differences between responses, including ideas of responses being ‘segmented’ to identify their structure.
        \\
        outliers
        & Identifying outliers or unique features.
        \\
        diversity
        & Determining consistency or diversity across sets of responses. 
        \\

    \midrule
        
    \multicolumn{2}{l}{\textbf{Preferences about Interface Elements}} \\

        display
        & Preferences about viewing all or many responses at once.
        \\
        scroll
        & Preferences about needing to scroll to return to responses.
        \\
        options
        & Preferences about the ability to disable features.
        \\
        delineation
        & Preferences about delineation between prompt groups (e.g. responses to different prompt variations).
        \\
        visual learner
        & Preferences about learning or processing information visually.
        \\

    \midrule
        
    \multicolumn{2}{l}{\textbf{Elements of Reading Process}} \\

        speed
        & What made reading responses faster or slower.
        \\
        read all
        & Reading the entirety of groups of responses (as opposed to skimming).
        \\
        skim
        & Skimming groups of responses. 
        \\
    
    \midrule
        
    \multicolumn{2}{l}{\textbf{Cognitive Elements}} \\
        
        memory
        & Issues of working memory, forgetting response content or location, or needing to reread in order to recall response attributes.
        \\
        ease
        & Cognitive demand of different interface elements.
        \\
        overwhelm
        & Feelings of overwhelm or stress, especially in response to attempting to incorporate too much information at once.
        \\
        exhaustion
        & Feelings of exhaustion or “zoning out”.
        \\
        focus
        & Ability (or inability) to focus on specific responses or groups of responses.
        \\
        difficulty
        & Feelings of task difficulty, including not knowing how to start a task.
        \\
    
    \midrule
        
    \multicolumn{2}{l}{\textbf{Methods of Detecting Similarities and Differences}} \\

        confirmation
        & Performing “hypothesis testing” or otherwise confirming or verifying an idea.
        \\
        comparison
        & Directly comparing responses by having them nearby or side by side.
        \\
        absent color
        & Making use of unhighlighted text segments.
        \\
        
    \midrule
        
    \multicolumn{2}{l}{\textbf{Feature Accuracy and Understanding}} \\

        accuracy
        & Determining how accurate or trustworthy different features are. 
        \\
        not understanding
        & Not understanding how a feature worked or why it performed a certain way.
        \\


  \bottomrule
\end{tabular}

